Learning and Sampling of Atomic Interventions from Observations

We study the problem of efficiently estimating the effect of an intervention on a single variable (atomic interventions) using observational samples in a causal Bayesian network. Our goal is to give algorithms that are efficient in both time and sample complexity in a non-parametric setting. Tian and Pearl (AAAI `02) have exactly characterized the class of causal graphs for which causal effects of atomic interventions can be identified from observational data. We make their result quantitative. Suppose P is a causal model on a set $\vec{V}$ of n observable variables with respect to a given causal graph G with observable distribution $P$. Let $P_x$ denote the interventional distribution over the observables with respect to an intervention of a designated variable X with x. Assuming that $G$ has bounded in-degree, bounded c-components ($k$), and that the observational distribution is identifiable and satisfies certain strong positivity condition, we give an algorithm that takes $m=\tilde{O}(n\epsilon^{-2})$ samples from $P$ and $O(mn)$ time, and outputs with high probability a description of a distribution $\hat{P}$ such that $d_{\mathrm{TV}}(P_x, \hat{P}) \leq \epsilon$, and: 1. [Evaluation] the description can return in $O(n)$ time the probability $\hat{P}(\vec{v})$ for any assignment $\vec{v}$ to $\vec{V}$ 2. [Generation] the description can return an iid sample from $\hat{P}$ in $O(n)$ time. We also show lower bounds for the sample complexity showing that our sample complexity has an optimal dependence on the parameters $n$ and $\epsilon$, as well as if $k=1$ on the strong positivity parameter.

==> doCcomp.tex <==
\subsection{Learning Interventions on c-Components}
\cref{lem:imp} together with the Bayes net learning algorithm also gives us a way to learn the joint distribution on a subset of  c-components when the remaining observable variables are intervened (assuming certain strong positivity condition), which we will use.  

%{\bf The following lemma has to be rewritten. Also the proof needs to be elaborated: Vinod}

%%%%%% ICML Version of the Lemma Ignored
\ignore{
\begin{lemma}\label{lem:learnComp}
Let ${\cal S} \subseteq \{\vec{S}_1,\dots,\vec{S}_{\ell}\}$ be any fixed set of c-components of $G$. Let $\vec{Y}$ be the set of vertices in ${\cal S}$ and $\bar{\vec{Y}}=\vec{V}\setminus \vec{Y}$. Let $\bar{\vec{y}}$ be any assignment of $\bar{\vec{Y}}$ and ${\bar{\vec{y}}_{\mathrm{Pa}}}$ be the restriction $\bar{\vec{y}}_{\Pa^{-}(\vec{Y})}$. Suppose $P({\bar{\vec{y}}_{\mathrm{Pa}}})\ge \alpha$. Then, $P_{\bar{\vec{y}}}(\vec{Y})=P_{{\bar{\vec{y}}_{\mathrm{Pa}}}}(\vec{Y})$ can be learnt to $\dtv$ distance $\leq\epsilon$ using $m=\tilde{O}(\log {1\over \delta}|\Sigma|^{kd+k+1}|\vec{Y}|/\alpha\epsilon^2)$ samples and $O(m|\vec{Y}||\Sigma|^{kd+k+1})$ time with probability $1-\delta$.
\end{lemma}
}

\begin{theorem}\label{lem:learnComp}
Let ${\cal S} \subseteq \{\vec{S}_1,\dots,\vec{S}_{\ell}\}$ be any fixed set of c-components of an ADMG $G$ on vertex set $[n]$ with maximum in-degree $d$ and maximum c-component size $k$. Let $\vec{Y}$ be the set of vertices in ${\cal S}$ and $\overline{\vec{Y}}=\vec{V}\setminus \vec{Y}$. Let $\overline{\vec{y}}$ be any assignment of $\overline{\vec{Y}}$ and ${\overline{\vec{y}}_{1}}$ be the restriction $\overline{\vec{y}}_{\Pa^{-}(\vec{Y})}$. For every $V_i \in \vec{Y}$ let $\vec{Z}_i \subseteq \Pa^{+}(\vec{Y})$ be its effective parents from~\cref{eqn:obsfactor}. \ignore{Suppose $P({\overline{\vec{y}}_{1}})\ge \alpha$.} Then, 
\begin{enumerate}
\item $P_{\overline{\vec{y}}}(\vec{Y})=P_{{\overline{\vec{y}}_{1}}}(\vec{Y})= \prod_{V_i\in \vec{Y}} P(V_i \mid \vec{Z}_i \cap \vec{Y},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})$.
\end{enumerate}

For any $\eps, \delta \in (0,1)$ $P_{\overline{\vec{y}}}$ can be learnt as a bayes net $\hat{P}$ according to the above factorization such that 
$\dtv(P_{\overline{\vec{y}}},\hat{P})\allowbreak\le \epsilon$ with probability $ \geq 1-\delta$ using $m$ samples and $O(m|\vec{Y}||\Sigma|^{kd+k+1}+|\vec{Y}|^2|\Sigma|^{2kd+2k+2}\epsilon^{-2}{\log^3 {\delta}^{-1}})$ time, where $m=$
\begin{enumerate}[resume]
\item  $O(|\vec{Y}||\Sigma|^{kd+k+1}\log (|\vec{Y}||\Sigma|^{kd+k})\log {\delta^{-1}}\alpha^{-|\Pa^{-}(\vec{Y})|}\epsilon^{-2})$, if $P$ is $\alpha$-strongly positive w.r.t. $\Pa^+(\overline{\vec{Y}})$
\item $O(|\vec{Y}||\Sigma|^{kd+d+1}\log {\delta^{-1}}\alpha^{-1}\epsilon^{-2})$, if $P$ is $\alpha$-strongly positive w.r.t. $\Pa^{+}(\vec{Y})$
\end{enumerate}
\end{theorem}
We break the proof of~\cref{lem:learnComp} into 4 parts for the ease of presentation. The first part contains the proof of the first claim. The next two parts prove the second and third came for $\delta=0.3$. We give the $1-\delta$ success probability algorithm in the final part of the proof.



\begin{proof}[Proof of~\cref{lem:learnComp} Part 1]
Follows from \cref{lem:imp} by considering $\mathcal{S}$ effectively a single c-component. We give a proof below for completeness. By definition $P_{\overline{\vec{y}}}(\vec{Y})$ is the distribution of $\mathcal{P}$ where $\overline{\vec{Y}}$ take the value $\overline{\vec{y}}$ with probability 1, their incoming edges are removed, and the remaining vertices follow the conditional probabilities of $\mathcal{P}$. In this bayes net, the marginal distribution on $\Pa^{+}(Y)$ can be factorized as $\prod_{V_i \in \Pa^{+}(Y)} P(V_i \mid \vec{Z}'_i)$ where $\vec{Z}'_i$ is the set of vertices before $V_i$ in the topological ordering of $\Pa^{+}(Y)$ according to $G$. For $V_i\in \Pa^{-}(Y)$ (new root nodes), we replace the terms $P(V_i=\overline{\vec{y}}_{V_i})$   by 1 and $P(V_i\neq\overline{\vec{y}}_{V_i})$  by 0. Finally we replace $\vec{Z}'_i$ by $\vec{Z}_i:=\vec{Z}'_i \cap \Pa^{+}(\vec{T}_i)$ as $V_i$ is independent of $\vec{Z}'_i\setminus\vec{Z}_i$ conditioned on $\vec{Z}_i$, taking into account the hidden variables' confounding. Clearly, in this factorization the values $\overline{\vec{y}} \setminus {\overline{\vec{y}}_{1}}$ does not matter. Also note that $\vec{Z}_i$ coincides with that in~\cref{eqn:obsfactor} because c-component structure of $\vec{Y}$ is unchanged and the topological ordering of $G$ remains the same.
\end{proof}

For the last two parts we use a KL local subadditivity result for bayes nets from Canonne et al.~\cite{Canonne}. For a bayes net $P$, a vertex $i$ and an assignment $\vec{a}$ to its parents, let $\Pi[i,\vec{a}]$ denote the event that the parents of a variable $i$ is $\vec{a}$ and let $P(i\mid \vec{a})$ denote the conditional distribution of variable $i$ when its parents are $\vec{a}$.
\begin{theorem}[\cite{Canonne}]\label{thm:bnadd}
Let $P, Q$ be two bayes nets over a common graph. Then $\dkl(P,Q)\le \sum_i \sum_{\vec{a}} P[\Pi[i,\vec{a}]]\; \dkl(P(i\mid\vec{a}),Q(i\mid\vec{a}))$
\end{theorem}
We apply the above result in the bayes net $P_{\overline{\vec{y}}_1}$ for the variables $V_i\in \vec{Y}$ and their effective parents $\vec{Z}_i$. We also need the following result for learning an unknown distribution in $\dkl$ distance.
\begin{theorem}[\cite{pmlr-v40-Kamath15}]\label{thm:laplacelearn}
Let $D$ be an unknown distribution over $[m]$. Suppose we take $z$ samples from $D$ and define the add-1 empirical distribution $D'(i)=(z_i+1)/(z+m)$ where $z_i$ is the number of occurrences of item $i$. Then $\ex{\dkl(D,D')}\le (m-1)/(z+1)$.
\end{theorem}

We first show the following relationship between the observational and interventional probabilities.
\begin{lemma}\label{lem:obsdo}
Suppose $P$ is $\alpha$-strongly positive w.r.t. $\Pa^+(\overline{\vec{Y}})$. Then for any assignment $\vec{y}$ to $\vec{Y}$ and $\overline{\vec{y}}_1$ to $\Pa^{-}(\vec{Y})$, $P(\overline{\vec{y}}_1,\vec{y})\ge \alpha^{|\Pa^{-}(\vec{Y})|} P_{\overline{\vec{y}}_1}(\vec{y})$
\end{lemma}
\begin{proof}
Let $\vec{c}$ be an assignment to $\vec{V} \setminus \Pa^{+}(\vec{Y})$. Let $\vec{v}=\vec{c}\circ \overline{\vec{y}}_1 \circ \vec{y}$
\begin{align*}
P(\vec{c},\overline{\vec{y}}_1,\vec{y}) &= \prod_{i=1}^n P(v_i \mid \vec{v}_{\vec{Z}_i})\\
&= \prod_{i \in \vec{Y}} P(v_i \mid \vec{v}_{\vec{Z}_i}) \prod_{i\in  \vec{V}\setminus \Pa^{+}(\vec{Y})} P(v_i \mid \vec{v}_{\vec{Z}_i}) \prod_{i\in \Pa^{-}(\vec{Y})} P(v_i \mid \vec{v}_{\vec{Z}_i})\\
&\ge \prod_{i \in \vec{Y}} P(v_i \mid \vec{v}_{\vec{Z}_i}) \prod_{i\in  \vec{V}\setminus \Pa^{+}(\vec{Y})} P(v_i \mid \vec{v}_{\vec{Z}_i}) \prod_{i\in \Pa^{-}(\vec{Y})} P(v_i, \vec{v}_{\vec{Z}_i})\\
&\ge \prod_{i \in \vec{Y}} P(v_i \mid \vec{v}_{\vec{Z}_i}) \prod_{i\in  \vec{V}\setminus \Pa^{+}(\vec{Y})} P(v_i \mid \vec{v}_{\vec{Z}_i}) \alpha^{|\Pa^{-}(\vec{Y})|}
\end{align*}
The third line follows from $P(A\mid B)\ge P(A\mid B)P(B) = P(AB)$ for any two events $A$ and $B$. The fourth line follows since for every $i\in \Pa^{-}(\vec{Y})$, $\vec{Z}_i \cup \{V_i\} \subseteq \Pa^{+}(T_i) \subseteq \Pa^+(\overline{\vec{Y}})$ where $T_i$ is the c-component of $V_i$ and $P$ is $\alpha$-strongly positive w.r.t $\Pa^+(\overline{\vec{Y}})$.

We next take summation over all assignments $\vec{c}$. Variables in $\vec{V}\setminus\Pa^{+}(\vec{Y})$ do not appear in the right side of $\mid$ in the factors $\prod_{i \in \vec{Y}} P(v_i \mid \vec{v}_{\vec{Z}_i})$. Hence they can be marginalized out one after another in the topological order to give $\sum_{\vec{c}} \prod_{i\in  \vec{V}\setminus \Pa^{+}(\vec{Y})} P(v_i \mid \vec{v}_{\vec{Z}_i})=1$. Note that when $\Pa^{-}(\vec{Y})=\overline{\vec{y}}_1$, $\prod_{i \in \vec{Y}} P(v_i \mid \vec{v}_{\vec{Z}_i})=P_{\overline{\vec{y}}_1}(\vec{y})$. We get $P(\overline{\vec{y}}_1,\vec{y}) \ge \alpha^{|\Pa^{-}(\vec{Y})|} P_{\overline{\vec{y}}_1}(\vec{y})$.

\end{proof} 

\begin{figure}
\begin{algorithm}[H]
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Samples from $P$, parameters $m,t$}
\Output{A bayes net $\hat{P}$ on the same graph as of $P_{\overline{\vec{y}}_1}$}
Get $m$ samples from $P$\;
\For{every vertex $V_i\in \vec{Y}$}{
\For{every fixing $\vec{Z}_i \cap \vec{Y}=\vec{a}$}{
$N_{i,\vec{a}} \gets$ the number of samples where $V_i$'s parents are $\vec{a}\circ \overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}$\;
\eIf{$N_{i,\vec{a}} \ge t$}{
$\hat{P}(V_i\mid \vec{a}, \overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}) \gets$ the add-1 empirical distribution (see~\cref{thm:laplacelearn}) at node $i$ in the subset of samples where $V_i$'s parents are $\vec{a}\circ \overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}$\;
}{
$\hat{P}(V_i\mid \vec{a}, \overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}) \gets$ uniform distribution over $\Sigma$\;
} 
}
}
\caption{Learning $P_{\overline{\vec{y}}_1}$}
\label{algo:bn}
\end{algorithm}
\end{figure}

\begin{proof}[Proof of~\cref{lem:learnComp} Part 2 for $\delta=0.3$]
We use~\cref{algo:bn} to learn $P_{\overline{\vec{y}}_1}$ with the parameters $m=16|\vec{Y}||\Sigma|^{kd+k+1}\log (|\vec{Y}||\Sigma|^{kd+k})/\alpha^{|\Pa^{-}(\vec{Y})|}\epsilon^2$ and $t=\log (|\vec{Y}||\Sigma|^{kd+k})$. We get from~\cref{thm:bnadd}:
\begin{equation}\label{eqn:bncase1}
\dkl(P_{\overline{\vec{y}}_1},\hat{P})\le \sum_i \sum_{\vec{a}} P_{\overline{\vec{y}}_1}[\vec{Z}_i \cap \vec{Y}=\vec{a}]\; \dkl(P(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}),\hat{P}(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}))
\end{equation}
 since $P_{\overline{\vec{y}}}(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})=P_{\overline{\vec{y}}_1}(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})=P(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})$.

We partition the set of tuples $(i,\vec{a})$ into two parts: {\em heavy} if $P_{\overline{\vec{y}}}[\vec{Z}_i \cap \vec{Y}=\vec{a}]\ge \epsilon^2/(8|\vec{Y}||\Sigma|^{kd+k+1})$ and {\em light} otherwise. We get $P(\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}},\vec{a}) \ge P({\overline{\vec{y}}_{1}},\vec{a}) \ge \alpha^{|\Pa^{-}(\vec{Y})|} P_{\overline{\vec{y}}_1}[\vec{Z}_i \cap \vec{Y}=\vec{a}]$, the last step by marginalizing out $\vec{y}\setminus \vec{a}$ in~\cref{lem:obsdo}.
Consider the event ``all heavy tuples satisfy $N_{i,\vec{a}}\ge 8|\vec{Y}||\Sigma|^{kd+k+1} P_{\overline{\vec{y}}}[\vec{Z}_i \cap \vec{Y}=\vec{a}](\vec{a})t/\epsilon^2$''. It is easy to see from
Chernoff and union bounds that this event holds with 19/20 probability for a large enough $|Y|$. Hence for the rest of the
argument, we condition on this event. In this case, all heavy items satisfy $N_{i,\vec{a}} \ge t$. We have from~\cref{thm:laplacelearn}:

\begin{itemize}
\item For all heavy $(i,\vec{a})$ $\ex{\dkl(P(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}),\hat{P}(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})} \le {\epsilon^2(|\Sigma|-1) \over 8|\vec{Y}||\Sigma|^{kd+k+1} P_{\overline{\vec{y}}_1}(\vec{a})t}$
\item For any light items which satisfy $N_{i,\vec{a}} \ge t$ $\ex{\dkl(P(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}),\hat{P}(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})} \le {(|\Sigma|-1) \over t}$
\item Items which do not satisfy $N_{i,\vec{a}} \ge t$ must be light for which we have $\ex{\dkl(P(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}),\hat{P}(i\mid\vec{a},
\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})} \le \sum_{\sigma\in \Sigma} P(i=\sigma\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})\ln({|\Sigma|P(i=\sigma\mid
\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})}) = \sum_{\sigma\in \Sigma} P(i=\sigma\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})\allowbreak\ln |\Sigma|-
H(P(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}})) \le \ln |\Sigma|$, where $H(\cdot) \ge 0$ is the Shannon entropy function.
\end{itemize}

Together we get each summand in the r.h.s of~\cref{eqn:bncase1} is at most ${\epsilon^2\over 8|\vec{Y}||\Sigma|^{kd+k+1}}\max\{{(|\Sigma|-1) \over t},\ln |\Sigma|\}$. Since there are at most $|\vec{Y}||\Sigma|^{kd+k}$ summands, we get $\ex{\dkl(P_{\overline{\vec{y}}},\hat{P})} \le \epsilon^2/8$. From Markov's inequality we get $\dkl(P_{\overline{\vec{y}}},\hat{P}) \le \epsilon^2/2$ except 1/4 probability. In this case, Pinsker's inequality gives $\dtv(P_{\overline{\vec{y}}},\hat{P}) \le \epsilon$, the total error probability being at most 0.3.
\end{proof}

\begin{proof}[Proof of~\cref{lem:learnComp} Part 3 for $\delta=0.3$]
We use~\cref{algo:bn} to learn $P_{\overline{\vec{y}}_1}$ with the parameters $m=16|\vec{Y}||\Sigma|^{kd+d+1}/\alpha\epsilon^2$ and $t=8|\vec{Y}||\Sigma|^{kd+d+1}/\epsilon^2$. We get from~\cref{eqn:bncase1}:
\begin{equation}\label{eqn:bncase2}
\dkl(P_{\overline{\vec{y}}},\hat{P})\le \sum_i \sum_{\vec{a}} \dkl(P(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}),\hat{P}(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}))
\end{equation}
 since $P_{\overline{\vec{y}}_1}[\vec{Z}_i \cap \vec{Y}=\vec{a}]\le 1$.

For every vertex $i$ and every assignment $\vec{a}$ to $\vec{Z}_i \cap \vec{Y}$, $P[\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}] \ge \alpha$ by assumption since $\vec{Z}_i \subseteq \Pa^{+}(\vec{Y})$. Hence $N_{i,\vec{a}} \ge t$ for every $i, \vec{a}$ by Chernoff and union bounds except 19/20 probability. From~\cref{thm:laplacelearn} we get 
$\ex{\dkl(P(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}),\hat{P}(i\mid\vec{a},\overline{\vec{y}}_{\vec{Z}_i \setminus \vec{Y}}))} \le (|\Sigma|-1)/t < \epsilon^2/8|\vec{Y}||\Sigma|^{kd+k}$. Taking the summation and applying Markov's and Pinsker's inequalities we get $\dtv(P_{\overline{\vec{y}}_1},\hat{P}) \le \epsilon$ with probability at least 0.7.
\end{proof}

\begin{proof}[Proof of~\cref{lem:learnComp} Parts 2 and 3 for failure probability $\le \delta$]
We invoke the following result given in~\cite{BGMV20}, which takes the 0.7 success probability algorithms designed above and gives a $(1-\delta)$ success probability algorithm.
\begin{theorem}[Theorem 2.9 in~\cite{BGMV20} restated]
Fix any $0<\epsilon,\delta<1$.
Suppose we are given an algorithm that learns an unknown bayes net $P$ over $\Sigma^N$ on a graph $G$ with indegree $\le \Delta$ as a bayes net $\hat{P}$ on $G$ such that $\dtv(P,\hat{P})\le \epsilon$ with probability at least 0.7 using $m(\epsilon)$ samples and $t(\epsilon)$ time. Then we can output a distribution $P'$ on $G$ such that $\dtv(P,P')\le \epsilon$ with probability at least $(1-\delta)$ using $O(m(\epsilon/4)\log {1\over \delta})$ samples and $O(t(\epsilon/4)\log {1\over \delta}+|\Sigma|^{2\Delta} N^2\epsilon^{-2}\log^3 {1\over \delta})$ time.
\end{theorem} 
\end{proof}

\ignore{
$P_{\overline{\vec{y}}}(\vec{Y})=P_{{\overline{\vec{y}}_{1}}}(\vec{Y})$ follows from the fact that the intervention $\overline{\vec{y}}_{\mathrm{Pa}}$ blocks any other interventions since these are the immediate parents of $\vec{Y}$ in $G$. 
An informal argument to show $P_{\overline{\vec{y}}}(\vec{Y})$ is identifiable implicitly follows from \cref{lem:imp}. We can put dummy bidrected edges to make $\vec{S}$ a single c-component and apply part (ii) of \cref{lem:imp}. In the resulting factorization the terms are of the form $P(v_i \mid v_{[i-1]})$. But then we can only keep the subset of variables of $v_{[i-1]}$ which are from the c-component of $v_i$ and the parents of this c-component, and remove the rest using conditional independence (blocking), since the dummy bidirected edges are not affecting.

Hence for a fixed assignment ${\overline{\vec{y}}_{1}}$, the factorization of the joint distribution $P_{\overline{\vec{y}}}(\vec{Y})$ consists of the product of only the terms $P(V_i\mid \vec{Z}_i)$ for every $i \in \vec{Y}$, where the set $\vec{Z}_i$ has at most $kd+k$ variables among which the variables coming from $\Pa^{-}(\vec{Y})$ are fixed to ${\overline{\vec{y}}_{1}}$. More formally this fact can be proven by closely following the proof of \cref{lem:imp}.

It follows by comparing the above factorization of $P_{\overline{\vec{y}}}(\vec{Y})$ and the factorization of $P(\vec{V})$ from \cref{lem:imp} that the conditional samples from $P(\vec{V})$ with $\Pa^{-}(\vec{Y})={\overline{\vec{y}}_{1}}$ is according to the distribution $P_{\overline{\vec{y}}}(\vec{Y})$. Moreover $P_{\overline{\vec{y}}}(\vec{Y})$ is a Bayes net with degree at most $kd+k$ as we discussed in the previous paragraph. From~\cref{thm:bnlearning} $m'=O(\log {1\over \delta}|\Sigma|^{kd+k+1}|\vec{Y}|\log (|\vec{Y}||\Sigma|^{kd+k+1})/\epsilon^2)$ conditional samples and processing time $O(m'|\vec{Y}||\Sigma|^{kd+k+1})$ is enough to learn in $\dtv$ distance $\le \eps$. 
The result follows by observing $O(m'/\alpha)$ samples from $P$ are enough to give $m$ conditional samples except for probability $\le \delta$. 

}

==> eval.tex <==
%!TEX root=MAIN.tex
\subsection{Evaluation of $P_x$}\label{subsec:eval}

%\begin{figure}
%\includegraphics[scale=0.5]{alg1}

\begin{algorithm}[H]
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Sample access to $P$}
\Output{Evaluator for $P_x$}
\For{every assignment $\vec{a}$ of $\vec{A}=\vec{S}_1\setminus \{X\}$}{
$S\gets$ Draw $\tilde{\Theta}(n|\Sigma|^{kd+3k+1}/\alpha^k\epsilon^2)$ samples from $P$\;
$R'_{\vec{a}}(\vec{B},\vec{C}) \gets $Learn $P_{\vec{a}\circ x}(\vec{B}, \vec{C})$ by~\cref{lem:learnComp} Part 2 in using $S$\;
}

\For{every assignment $\vec{b}$ to $\vec{B}=\Pa^-(\vec{S}_1)$}{
$S\gets$ Draw $\tilde{\Theta}(k|\Sigma|^{kd+3k+1}/\alpha\epsilon^2)$ samples from $P$\;
$M'_{\vec{b}}(\vec{S}_1) \gets $Learn $P_{\vec{b}}(\vec{S}_1)$ by~\cref{lem:learnComp} Part 3 using $S$\;
}

\Return{a function that, on input an assignment $\vec{w}=\vec{a}\circ \vec{b} \circ \vec{c}$ to $\vec{W} = \vec{V}\setminus \{X\}$, outputs $(\sum_{x' \in \Sigma} M'_{\vec{b}}(\vec{a},x'))\cdot R'_{\vec{a}}(\vec{b},\vec{c})$\;}
\caption{Algorithm to output evaluator for $P_x$. For notations, please refer to~\cref{subsec:eval}}
\label{algo:Eval}
\end{algorithm}
%\end{figure}
\begin{proof}[Proof of \cref{thm:learn1}]

In view of \cref{thm:tp}, for an assignment $\vec{w}=\vec{a}\circ \vec{b} \circ \vec{c}$ ($\vec{w}_{\vec{A}}=\vec{a}$, $\vec{w}_{\vec{B}}=\vec{b}$, $\vec{w}_{\vec{C}}=\vec{c}$) to $\vec{V} \setminus \{x\}$ let us define $M$ and $R$ so that $P_x(\vec{w})=M(\vec{w})R(\vec{w})$:
$$M(\vec{w}) = P_{\vec{w}_{\vec{B}}}(\vec{w}_{\vec{A}}) = \sum_{x'}P_{\vec{w}_{\vec{B}}}(\vec{w}_{\vec{A}} \circ x') = \sum_{x' \in \Sigma}Q_{\vec{S}_1}(\vec{w}\circ x')$$\\[-8pt]
$$R(\vec{w}) = P_{\vec{w}_{\vec{A}}\circ x}(\vec{w}_{\vec{B} \cup \vec{C}}) = \prod_{j=2}^\ell Q_{\vec{S}_j}(\vec{w}\circ x).$$

Our strategy will be to approximate $R$ and $M$ separately as $R'$ and $M'$, and then output their product. See~\cref{algo:Eval}.  

For every assignment $\vec{a}$ to $\vec{A}$, let $R_{\vec{a}}$ denote the partial function of $R$ for those $\vec{w}$ such that $\vec{w}_{\vec{A}} = \vec{a}$. Note that we can interpret $R_{\vec{a}}$ as a probability distribution on $\vec{B} \cup \vec{C}$, thus $R(\vec{a},\vec{b},\vec{c})=R_{\vec{a}}(\vec{b},\vec{c})$. Invoking \cref{lem:learnComp} part 2 and using \cref{ass:bal}, for every $\vec{a}$, we can learn an $R'_{\vec{a}}$ such that $\dtv(R'_{\vec{a}}, R_{\vec{a}})<\epsilon/2|\Sigma|^k$, using $\tilde{O}(|\Sigma|^{5kd} n/\alpha^k \epsilon^2)$ samples.

For a particular assignment $\vec{b}$ to $\vec{B}$, let $M_{\vec{b}}$ denote the partial function of $M$ for those $\vec{w}$ such that $\vec{w}_{\vec{B}} = \vec{b}$. We can interpret $M_{\vec{b}}$ as a probability distribution on $\vec{A}$, thus $M(\vec{a},\vec{b},\vec{c})=M_{\vec{b}}(\vec{a})$. We learn the distribution on all of $\vec{S}_1$ and then take its marginal on $\vec{A}$. Again, we invoke \cref{lem:learnComp} part 3 and \cref{ass:bal}, so that for every $\vec{b}$, we learn an $M'_{\vec{b}}$ that is within $\epsilon/2|\Sigma|^k$ TV distance of $M_{\vec{b}}$.

Finally, we use \cref{lem:dtvineq} below to combine the two estimates to obtain an estimate $P'_x(\vec{w}):=M'(\vec{w})R'(\vec{w})$.

\begin{lemma}\label{lem:dtvineq}
Suppose for all assignments $\vec{b}$ to $\vec{B}$, $\dtv(M_{\vec{b}}(\vec{A}),M'_{\vec{b}}(\vec{A})) \le \epsilon_1$ 
and for all assignments $\vec{a}$ to $\vec{A}$, $\dtv(R_{\vec{a}}(\vec{B},\vec{C}),R'_{\vec{a}}(\vec{B},\vec{C})) \le \epsilon_2$. 
Then $\sum_{\vec{w} \in \Sigma^{n-1}} |P_x(\vec{w})-P'_x(\vec{w})|\le |\Sigma|^{k}(\epsilon_1+\epsilon_2)$.
\end{lemma}
\begin{proof}
{\allowdisplaybreaks
\begin{align*}
\sum_{\vec{w}} |P_x(\vec{w})-P'_x(\vec{w})| &= \sum_{\vec{w}} |M(\vec{w})R(\vec{w})-M'(\vec{w})R'(\vec{w})|\\
&=\sum_{\vec{w}} |M(\vec{w})R(\vec{w})- M(\vec{w})R'(\vec{w})+M(\vec{w})R'(\vec{w}) - M'(\vec{w})R'(\vec{w})|\\
&\le \sum_{\vec{w}} [M(\vec{w})|R(\vec{w})- R'(\vec{w})|+|M(\vec{w})- M'(\vec{w})|R'(\vec{w})]
\end{align*}
We upper bound each of the above two terms separately. We break $\vec{w}=\vec{a}\circ \vec{b} \circ \vec{c}$ corresponding to $\vec{A}, \vec{B}$ and $\vec{C}$ respectively.
\begin{align*}
\sum_{\vec{a},\vec{b},\vec{c}} |M_{\vec{b}}(\vec{a})-M'_{\vec{b}}(\vec{a})|R_{\vec{a}}(\vec{b}, \vec{c}) &= \sum_{\vec{b},\vec{c}} (\sum_{\vec{a}} |M_{\vec{b}}(\vec{a})-M'_{\vec{b}}(\vec{a})|R_{\vec{a}}(\vec{b}, \vec{c}))\\
&\le \sum_{\vec{b},\vec{c}} (\sum_{\vec{a}} |M_{\vec{b}}(\vec{a})-M'_{\vec{b}}(\vec{a})|)(\sum_{\vec{a}} R_{\vec{a}}(\vec{b},\vec{c}))\\
&\le \sum_{\vec{b},\vec{c}}\epsilon_1\sum_{\vec{a}} R_{\vec{a}}(\vec{b},\vec{c})\\
&\le \epsilon_1 |\Sigma|^k \\
\sum_{\vec{w}} M(\vec{w})|R(\vec{w})-R'(\vec{w})| 
&\le \sum_{\vec{w}} |R(\vec{w})-R'(\vec{w})|\\
&\le \sum_{\vec{a}} \epsilon_2\\
& \le \epsilon_2 |\Sigma|^k
\end{align*}}
\end{proof}
Finally we claim $P'_x$ is a valid distribution satisfying $\sum_{\vec{w}} P'_x(\vec{w})=\sum_{\vec{w}} M'(\vec{w})R'(\vec{w})$ $=1$. In the bayes net factorization of $M'(\vec{w})R'(\vec{w})$ for every variable $V_j\in \vec{V}\setminus \{X\}$ we have exactly one term in either the Bayes nets $M'$ as $M'(w_j\mid \vec{w}_{\Pa(V_j)})$ or in $R'$  as $R'(w_j\mid \vec{w}_{\Pa(V_j)})$ resp.. We first marginalize out the sink nodes of $G$ using $\sum_{w_j \in \Sigma} M'(w_j\mid \vec{w}_{\Pa(\{j\})})=1$ or $\sum_{w_j \in \Sigma} R'(w_j\mid \vec{w}_{\Pa(\{j\})})=1$ as appropriate. Then we marginalize out the nodes which only have edges to the sink nodes and so on in the reverse topological order. When the vertex $X$'s turn comes we marginalize out $\sum_{x'\in \Sigma}$ as it appears inside $M'$.
\end{proof}

\ignore{
\begin{remark}
We claim $\sum_{\vec{w}} P'_x(\vec{w})=\sum_{\vec{w}} M'(\vec{w})R'(\vec{w})$ $=1$. In this factorization every variable $w_j$ appears exactly once in either of the Bayes nets $M'$ or $R'$ as $Pr(w_j\mid \vec{Z}_j)$. We first marginalize out the sink nodes of $G$ to get $\sum_{w_j \in \Sigma} Pr(w_j\mid \vec{Z}_j)=1$. Then we marginalize out the nodes which only have edges to the sink nodes and so on in the reverse topological order. When the vertex $X$'s turn comes we marginalize out $\sum_{x'}$ as it appears inside $M'$.
\end{remark}
}

==> misc.tex <==
\section{Proof of Lemma \ref{lem:dtvineq}}

==> samp.tex <==
%!TEX root=MAIN.tex
\subsection{Generation of $P_x$}
\begin{proof}[Proof of \cref{thm:learn2}]
From \cref{thm:learn1}, we obtain a distribution $P'_x$ such that $\dtv(P_x,P'_x)\le \epsilon$ and $P'_x(\vec{w})$ for an assignment $\vec{w}=\vec{a}\circ \vec{b} \circ \vec{c}$ ($\vec{w}_{\vec{A}}=\vec{a}$, $\vec{w}_{\vec{B}}=\vec{b}$, $\vec{w}_{\vec{C}}=\vec{c}$) to $\vec{V}\setminus \{X\}$ can be evaluated efficiently as $P'_x(\vec{w})=M'_{\vec{b}}(\vec{a})R'_{\vec{a}}(\vec{b},\vec{c})$, where $M'$ and $R'$ are two collections of Bayes nets. $P'_x$  as stated above is not efficiently samplable. So, we give a third distribution $\hat{P}_x$ which can be sampled efficiently and satisfies $\dtv(\hat{P}_x,P_x)\le 7\epsilon$. The subsequent discussion is computational where we work with the distribution $P'_x$ and don't need to consider $P$.

We write $R'_{\vec{a}}(\vec{b},\vec{c})=R'_{\vec{a}}(\vec{b})R'_{\vec{a}}(\vec{c}\mid\vec{ b})$ where $R'_{\vec{a}}(\vec{c}\mid \vec{b})$ is only defined for $R'_{\vec{a}}(\vec{b})\neq 0$. We write $P'_x(\vec{w})=M'_{\vec{b}}(\vec{a})R'_{\vec{a}}(\vec{b})\hat{R}_{\vec{a}}(\vec{c}\mid \vec{b})$. Note that $P'_x(\vec{a},\vec{b})=M'_{\vec{b}}(\vec{a})R'_{\vec{a}}(\vec{b})$ by marginalizing out $\vec{c}$ both sides. Hence we get $P'_x(\vec{w})=P'_x(\vec{a},\vec{b})R'_{\vec{a}}(\vec{c}\mid \vec{b})$.

Recall that $\vec{A}$ and $\vec{B}$ are small ($\leq k$ and $\leq kd$ resp.) while $\vec{C}$ is huge.
Our approach is to learn $P'_x(\vec{a},\vec{b})=M'_{\vec{b}}(\vec{a})R'_{\vec{a}}(\vec{b})$ as $\hat{P}_x(\vec{a},\vec{b})=M'_{\vec{b}}(\vec{a})\hat{R}_{\vec{a}}(\vec{b})$ and store it explicitly, while using rejection sampling for $R'_{\vec{a}}(\vec{c}\mid \vec{b})$. Our samplable distribution is defined as $\hat{P}_x(\vec{w})=\hat{P}_x(\vec{a},\vec{b})R'_{\vec{a}}(\vec{c}\mid \vec{b})$.
Sampling $R'_{\vec{a}}(\vec{c}\mid \vec{b})$ would require large enough probability mass for $R'_{\vec{a}}(\vec{b})$ which we ensure. If $R'_{\vec{a}}(\vec{b})=0$ we also make sure $\hat{P}_x(\vec{a},\vec{b})=0$. We make sure $\dtv(P'_x(\vec{A},\vec{B}),\hat{P}_x(\vec{A},\vec{B}))\le 6\epsilon$ which gives $\dtv(P'_x,\hat{P}_x)\le 6\epsilon$ since $R'_{\vec{a}}(\vec{c}\mid \vec{b})$ is unchanged.

Note that we already know $M'_{\vec{b}}(\vec{a})$ for every $\vec{a},\vec{b}$. Naively computing $R'_{\vec{a}}(\vec{b})$ would require an intractable marginalization. Instead, for every $\vec{a}$ we learn the distribution $R'_{\vec{a}}(\vec{B})$ as $\hat{R}_{\vec{a}}(\vec{B})$ upto $\epsilon/|\Sigma|^k$ distance in $\dtv$ by sampling from the known Bayes net $R'_{\vec{a}}(\vec{A},\vec{B})$. We use the empirical distribution of $\max\{m_1,m_2\}$ samples of $R'_{\vec{a}}(\vec{A},\vec{B})$ per $\vec{a}$, where $m_1=O((|\Sigma|^{kd+2k}+\log {|\Sigma|^{k}\over \delta})/\epsilon^2)$ and $m_2=O(|\Sigma|^{2kd+2k}\log {|\Sigma|^{kd+k}\over \delta}/\epsilon^2)$. $m_1$ samples make sure we learn $R'_{\vec{a}}(\vec{B})$ in $\dtv$ distance $\le \epsilon/|\Sigma|^k$ for all $\vec{a}$ except $\le\delta$ probability from a standard result. $m_2$ samples make sure if $0<R'_{\vec{a}}(\vec{b})\le \epsilon/|\Sigma|^{kd+k}$ for any $\vec{a},\vec{b}$, the empirical probability value $\hat{R}_{\vec{a}}(\vec{b})$ is at most $2\epsilon/|\Sigma|^{kd+k}$ except $\le\delta$ probability by Hoeffding's bound. Subsequently we set $\hat{R}'_{\vec{a}}(\vec{b}) =0$ for any $\vec{b}$ whose empirical probability is at most $2\epsilon/|\Sigma|^{kd+k}$ and add the surplus probability to other $\vec{b}$'s to make $\hat{R}_{\vec{a}}(\vec{B})$ a distribution, for every $\vec{a}$. This step takes $O(m_2|\Sigma|^k)$ time and satisfy $\dtv(R'_{\vec{a}}(\vec{B}),\hat{R}_{\vec{a}}(\vec{B}))\le 3\epsilon/|\Sigma|^k$ for every $\vec{a}$. This step also makes sure if $0<R'_{\vec{a}}(\vec{b})\le \epsilon/|\Sigma|^{kd+k}$ then $\hat{P}_x(\vec{a},\vec{b})=\hat{R}_{\vec{a}}(\vec{b})=0$ and if $R'_{\vec{a}}(\vec{b})=0$ then $\hat{P}_x(\vec{a},\vec{b})=\hat{R}_{\vec{a}}(\vec{b})=0$ as no samples with $\vec{B} = \vec{b}$ would turn up in this case.

We get $\sum_{\vec{a},\vec{b}} |\hat{P}_x(\vec{a},\vec{b})-P'_x(\vec{a},\vec{b})| =
\sum_{\vec{a},\vec{b}} M'_{\vec{b}}(\vec{a})|R'_{\vec{a}}(\vec{b})-\hat{R}_{\vec{a}}
(\vec{b})| \le \sum_a 3\epsilon/|\Sigma|^k \le 3\epsilon$. At this point one issue is $
\sum_{\vec{a},\vec{b}} \hat{P}_x(\vec{a},\vec{b})$ might not be 1, although it lies in 
$[1-3\epsilon,1+3\epsilon]$. So we compute  $\sum_{\vec{a},\vec{b}} \hat{P}_x(\vec{a},\vec{b})$ and scale appropriately to make $\hat{P}_x(\vec{A},\vec{B})$ a 
distribution which makes the $\dtv$ distance at most ${3\epsilon\over 1-3\epsilon}<6\epsilon$ for $\epsilon<1/6$.

From the triangle inequality, it follows $\dtv(P_x,\hat{P}_x)\le 7\epsilon$. To sample from $\hat{P}_x$ we first sample $\vec{a},\vec{b} \sim \hat{P}_x(\vec{A},\vec{B})$ which we explicitly store. Subsequently we sample from the conditional distribution $\hat{R}_{\vec{a}}(\vec{c}\mid \vec{b})$ using rejection sampling (sampling until a $\vec{b}$ is hit). Since we make sure any item in the support of $\hat{P}_x$ satisfy $R'_{\vec{a}}(\vec{b})>\epsilon/|\Sigma|^{kd+k}$, this step may need $O(|\Sigma|^{kd+k}\log {1\over \delta}/\epsilon)$ samples and $O(n|\Sigma|^{kd+k}\log {1\over \delta}/\epsilon)$ time from the Bayes net $R'_{\vec{a}}(\vec{A},\vec{B})$ per sample in the worst case to succeed with probability $1-\delta$.
 \end{proof}
